Littelmann path model for geometric crystals, Whittaker functions on Lie groups and Brownian motion

Generally speaking, this thesis focuses on the interplay between the representations of Lie groups and probability theory. It subdivides into essentially three parts. In a first rather algebraic part, we construct a path model for geometric crystals in the sense of Berenstein and Kazhdan, for complex semi-simple Lie groups. We will mainly describe the algebraic structure, its natural morphisms and parameterizations. The theory of total positivity will play a particularly important role. Then, we anticipate on the probabilistic part by exhibiting a canonical measure on geometric crystals. It uses as ingredients the superpotential for the flag manifold and a measure invariant under the crystal actions. The image measure under the weight map plays the role of Duistermaat-Heckman measure. Its Laplace transform defines Whittaker functions, providing an interesting formula for all Lie groups. Then it appears clearly that Whittaker functions are to geometric crystals, what characters are to combinatorial crystals. The Littlewood-Richardson rule is also exposed. Finally we present the probabilistic approach that allows to find the canonical measure. It is based on the fundamental idea that the Wiener measure will induce the adequate measure on the algebraic structures through the path model. In the last chapter, we show how our geometric model degenerates to the continuous classical Littelmann path model and thus recover known results. For example, the canonical measure on a geometric crystal of highest weight degenerates into a uniform measure on a polytope, and recovers the parameterizations of continuous crystals.

==> abstract.tex <==
\begin{abstract}

  At first sight, Pitman's 2M-X theorem is very odd as it expresses a linear combination of a Brownian motion and 
its one sided supremum as a Markov process. That result from probability theory has known far reaching extensions. Among its numerous generalizations, Matsumoto and Yor 
(\cite{bib:MY00-1, bib:MY00-2}) have exhibited a result that could be seen as a 'geometric' or non-zero temperature version 
of Pitman's theorem. As, for multidimensional extensions, the approach initiated by Biane, Bougerol and O'Connell 
(\cite{bib:BJ, bib:BBO, bib:BBO2}) is based on the intuition that such a structure in probability can appear only from the 
world of rigid structures, Algebra, and more specifically group theory.

Our goal is to identify a 'Pitman-type' Markov property in a geometric multidimensional (group-theoretic) framework. 
Matsumoto and Yor's result is interpreted as the $SL_2$ case, while the result by Bougerol and al. is interpreted as 
the 'cristalline' case.

On the way, this will shed a new light on many ubiquitous mathematical objects such as Kashiwara crystals and their geometric counterpart, geometric crystals introduced recently by Kazhdan and Berenstein. We will introduce a geometric version of the Littelmann path model, using integrals of exponential functionals. The quantum Toda equation naturally arises, and we give integral representations for its eigenfunctions, thanks to intertwining measures. A canonical measure on geometric crystals is constructed.  Its image through the weight map is the natural geometric counterparts of the continuous Duistermaat-Heckmann measure as it is naturally interpreted as a conditionnal distribution of weights.

\linebreak
{ \bf Keywords: } Total positivity, Geometric crystals, Geometric Littelmann path model, superpotential on $G/B$, Quantum Toda, Absolutely convergent integral representations for Whittaker functions, Brownian motion, Pitman 2M-X theorem, Matsumoto-Yor analogue, Pitman transforms, Beta-Gamma algebra identities.
\end{abstract}


==> quantum_toda_intro.tex <==
In the context of geometric crystals, we aim at identifying the canonical measure in a natural way. A fruitful idea is to consider the measure induced on crystals by uniform paths in a path model. In the discrete Littelmann path model, taking the uniform probability measure on finite paths induces the measure \ref{eqn:canonical_measure_discrete} on the generated crystal (see RSK correspondence for the Littelmann path model). In the continuous setting, the uniform measure on finite paths is replaced by the Wiener measure: a 'uniformly chosen path' is nothing but Brownian motion. It is the essence of \cite{bib:BBO2}. The geometric setting is also continuous by definition.\\

In this chapter, we study crystals generated by a Brownian motion $\Bc_t = \langle \left(W_{s} \right)_{ 0 \leq s \leq t}\rangle$ as random objects. By analogy with the Young tableaux growth one obtains in the classical RSK correspondence, one can think of $\Bc_t$ as an dynamical object growing with time. There are mainly two aspects in this description.\\
\begin{itemize}
 \item One can examine how the 'shape' of $B_t$ evolves with time, or more precisely the dynamics of its highest weight $\Lambda_t = hw\left(B_t\right)$ which encodes its isomorphism class as a geometric crystal. $\Lambda_t$ is a Markov process whose infinitesimal generator is given by a Doob transform of the quantum Toda Hamiltonian using one of its eigenfunctions, a Whittaker function.\\
 \item Second, we will examine the law of $\langle \left(W_{s} \right)_{ 0 \leq s \leq t}\rangle$ conditionally to its highest weight being $\lambda$. This probability measure on $\Bc(\lambda)$ is the correct candidate for being the canonical probability measure on a geometric crystal. Whittaker functions play the role of character and are defined by an equation similar to \ref{eqn:character_discrete}.\\
\end{itemize}

\section{On probability theory}
The usual framework is the probability triplet $( \Omega, \mathcal{A}, \mathbb{P})$ with $\Omega$ the sample space, $\mathcal{A}$ the set of events and $\mathbb{P}$ our working probability measure. \\

Equality in law between random variables or processes will be denoted$\stackrel{\mathcal{L}}{=}$. As such, the equality in law between two random variables $X$ and $Y$ is written $X \stackrel{\mathcal{L}}{=} Y$, and means the equality of their probability measures $\P_X = P_Y$.

\subsection*{Processes}
 From now on, the abbreviation 'BM' will be short for 'Brownian motion'. For every process $X$ (or even a deterministic path) taking its values in a Euclidian space, we will use the notation $X^{(\mu)}_t := X_t + \mu t$.
\subsection*{Laws}
By $\gamma_{\mu}$ for $\mu>0$ will denote a gamma law with parameter $\mu$ and ${ \bf e}_\mu$ stands for an exponential variable with parameter $\mu$.


\section{Introduction}
The approach finds its source in the classical potential theory and its probabilistic counterparts, which revolves around a central idea: Harmonic functions on a domain are given by integrating functions on the boundary against Brownian motion's exit law.\\

We consider the hypoelliptic Brownian motion $B_t(X^{(\mu)})$ on the solvable group, that is driven by a Euclidian Brownian motion $X^{(\mu)}$ with drift $\mu$ on $\afrak$. Whittaker functions can be seen as harmonic functions for this process having a certain invariance property. It is a standard idea in potential theory that any harmonic function is an integral over the 'exiting law' of the underlying random walk, here the hypoelliptic Brownian motion. This will be made precise in section \ref{section:poisson_boundary}. We are able to explicitly compute this boundary distribution in section \ref{section:conditionning_approach}, using inductively one dimensional results that were known to Matsumoto and Yor. Such results are reviewed beforehand in section \ref{section:review_matsumoto_yor}.\\
In the end, for $\mu$ in the Weyl chamber, Whittaker functions $\psi_\mu$ are defined simply as the integral of a character on $N$ over the exit law, giving an explicit integral formula different from the one by Jacquet. Through conditionning, Whittaker functions define a different exit law that is absolutely continuous w.r.t the original one and the conditionned BM to exit with this law is the Whittaker process, a Markov process. For arbitrary finite starting points, it is an approximation of the highest weight process. Finally, we will have to deal with two technicalities in order to provide complete proofs of theorems \ref{thm:highest_weight_is_markov} and \ref{thm:canonical_measure}.\\
\begin{itemize}
 \item Obtain the highest weight process by taking a starting point that is '$-\infty$' (section \ref{section:measure_concentration}).\\
 \item Extend the framework to arbitrary $\mu$ (section \ref{section:intertwined_markov_kernels}).
\end{itemize}



